LES of a classical hydraulic jump: Influence of modelling parameters on the predictive accuracy

Results from large-eddy simulations of a classical hydraulic jump at inlet Froude number 2 are reported. The computations are performed using the general-purpose finite-volume based code OpenFOAM, and the primary goal is to evaluate the influence of modelling parameters on the predictive accuracy, as well as establish associated best-practice guidelines. A benchmark simulation on a dense computational mesh is conducted, and good agreement with existing reference data is found. The remaining simulations cover different selections of modelling parameters: geometric vs algebraic interface capturing, three mesh resolution levels, four choices of the convective flux interpolation scheme. Geometric interface capturing leads to better accuracy but deteriorated numerical stability and increased simulation times. Interestingly, numerical dissipation is shown to systematically improve the results, both in terms of accuracy and stability. The densest of the three grids, which is twice as coarse as the grid used in the benchmark simulation, was found to be sufficient for faithfully reproducing all the considered quantities of interest. The recommendation is therefore to use this grid, geometric interface capturing, and a second-order upwind scheme for the convective fluxes.

==> texfiles/appendicies.tex <==
\section{The influence of spanwise domain length} \label{app:spanwise}

\section{The influence of surface tension} \label{app:surface_tension}

\section{Higher CFL number simulations} \label{app:cfl}
